Exploring the Robustness of In-Context Learning with Noisy Labels

Recently, the mysterious In-Context Learning (ICL) ability exhibited by Transformer architectures, especially in large language models (LLMs), has sparked significant research interest. However, the resilience of Transformers' in-context learning capabilities in the presence of noisy samples, prevalent in both training corpora and prompt demonstrations, remains underexplored. In this paper, inspired by prior research that studies ICL ability using simple function classes, we take a closer look at this problem by investigating the robustness of Transformers against noisy labels. Specifically, we first conduct a thorough evaluation and analysis of the robustness of Transformers against noisy labels during in-context learning and show that they exhibit notable resilience against diverse types of noise in demonstration labels. Furthermore, we delve deeper into this problem by exploring whether introducing noise into the training set, akin to a form of data augmentation, enhances such robustness during inference, and find that such noise can indeed improve the robustness of ICL. Overall, our fruitful analysis and findings provide a comprehensive understanding of the resilience of Transformer models against label noises during ICL and provide valuable insights into the research on Transformers in natural language processing. Our code is available at https://github.com/InezYu0928/in-context-learning.

==> A6_train_conv.tex <==
\section{Training convergence with noisy labels.} 

For each $\sigma$, we train the model with corresponding label noise distribution and plot the training loss curve in Figure~\ref{fig:training_loss} with each line representing a model. Still, we focus on the class of noisy linear functions $F=\{f_w | f_w(x) = w ^Tx +\epsilon, w \in R^d\}$, in $d=20$ dimensions. 
Similar to~\citep{garg2023transformers}, we used curriculum learning during training where we started from a low-dimensional space and gradually increased to 20. Note that the model associated with $\sigma_{train}=0.0$ represents the case of no-label noise, which is exactly the standard training setting. By inspecting the position of the convergence, it is clear that for small label noises ($\sigma<0.6$), the training is well converged and the final loss is very close to the standard training. Even in the case of large noise variance ($\sigma=0.6, 0.8, 1$), the training can still converge to a certain extent. The main difference between training with noise and without noise is at the beginning where the loss remains high even with the adoption of curriculum learning. However, curriculum learning still works well since all the models nearly converge at step 30k.


\begin{figure}[htbp]
\centering
\includegraphics[width=0.75\linewidth]{figs/training_loss.pdf}
\caption{The training loss for a standard-sized transformer with Gaussian noise of $\sigma_{train} \in \left \{ 0.0,0.2,0.4,0.6,0.8,1.0 \right \}$}
\label{fig:training_loss}
\end{figure}
